Improving CNN-based Planar Object Detection with Geometric Prior Knowledge

In this paper, we focus on the question: how might mobile robots take advantage of affordable RGB-D sensors for object detection? Although current CNN-based object detectors have achieved impressive results, there are three main drawbacks for practical usage on mobile robots: 1) It is hard and time-consuming to collect and annotate large-scale training sets. 2) It usually needs a long training time. 3) CNN-based object detection shows significant weakness in predicting location. We propose an improved method for the detection of planar objects, which rectifies images with geometric information to compensate for the perspective distortion before feeding it to the CNN detector module, typically a CNN-based detector like YOLO or MASK RCNN. By dealing with the perspective distortion in advance, we eliminate the need for the CNN detector to learn that. Experiments show that this approach significantly boosts the detection performance. Besides, it effectively reduces the number of training images required. In addition to the novel detection framework proposed, we also release an RGBD dataset and source code for hazmat sign detection. To the best of our knowledge, this is the first work of image rectification for CNN-based object detection, and the dataset is the first public available hazmat sign detection dataset with RGB-D sensors.

==> Tex_hjw/Discussion.tex <==
\section{Discussion}
% For rectification, we did some experiments with another rectification approach which generate one rectified image per plane, by applying an additional scaling matrix instead of translation. It turns out CNN detector is not robust enough to multiple scales, espically with such small training set. 

%TODO: The sentence looks wired, maybe change it later (jianxiong)
Unfortunately, the detection system does not run in real-time for now. This is due to the current implementation architecture only runs on a single thread. 

% In terms of detection speed for the system, it does not run in real-time so far due to current implementation architecture, but it can be easily optimized through parallelizing oeprations. 

% TODO: maybe add planar homography
% Alternative, when calculating H matrix, use the planar homography matrix. 

% \subsection{Future Work}
% In this work, we use planar objects (hazmat signs) as an example to show that homogaphy-based image rectification could be helpful for CNN-based backbone detector when dealing with RGB-D data. The main reason is that planar objects has a unique, well-defined canonical view, compared to general objects. However, it is feasible and interesting to extend the current work for more general object.


